Learning Language and Multimodal Privacy-Preserving Markers of Mood from Mobile Data

Mental health conditions remain underdiagnosed even in countries with common access to advanced medical care. The ability to accurately and efficiently predict mood from easily collectible data has several important implications for the early detection, intervention, and treatment of mental health disorders. One promising data source to help monitor human behavior is daily smartphone usage. However, care must be taken to summarize behaviors without identifying the user through personal (e.g., personally identifiable information) or protected (e.g., race, gender) attributes. In this paper, we study behavioral markers of daily mood using a recent dataset of mobile behaviors from adolescent populations at high risk of suicidal behaviors. Using computational models, we find that language and multimodal representations of mobile typed text (spanning typed characters, words, keystroke timings, and app usage) are predictive of daily mood. However, we find that models trained to predict mood often also capture private user identities in their intermediate representations. To tackle this problem, we evaluate approaches that obfuscate user identity while remaining predictive. By combining multimodal representations with privacy-preserving learning, we are able to push forward the performance-privacy frontier.

==> arxiv2021_Mobile Data/figures/SAL.tex <==
\begin{figure*}%
    \centering
    \vspace{-0mm}
    \includegraphics[width=0.9\textwidth]{images/SAL.pdf}
    \vspace{-2mm}
    \caption{Diagram of the \names\ algorithm learned via the (1) \textit{pretrain}, (2) \textit{selection}, and (3) \textit{addition} phases. Boxes with numbers denote which parameters are being optimized in the corresponding step. For example, in the \textit{addition} phase (3), \names\ optimizes parameters $\delta$ in $g(.;\delta)$. (2a) depicts identity-dependent dimensions $z_\textrm{id}$, which is a sparse vector of size $\text{dim} (z_\textrm{feat})$ whose nonzero values (colored purple) signify dimensions of the identity-dependent subspace in $z_\textrm{feat}$.\vspace{-4mm}}%
    \label{fig:sal}%
\end{figure*}

==> arxiv2021_Mobile Data/figures/overview.tex <==
\begin{figure}%
    \centering
    \vspace{-0mm}
    \includegraphics[width=\linewidth]{images/overview.pdf}
    \vspace{-4mm}
    \caption{Intensive monitoring of behaviors via adolescents' natural use of smartphones may help identify real-time predictors of mood in high-risk youth as a proxy for suicide risk. While smartphones provide a valuable data source spanning text, keystrokes, app usage, and geolocation, one must take care to summarize behaviors without revealing user identities through personal (e.g., personally identifiable information) or protected attributes (e.g., race, gender) to potentially adversarial third parties.\vspace{-4mm}}
    \label{fig:overview}
\end{figure}

==> arxiv2021_Mobile Data/figures/privacy_representations.tex <==
\begin{figure*}%
    \centering
    \vspace{-0mm}
    \subfloat[\centering \textsc{MLP} (without privacy-preserving)]{{\includegraphics[width=5.5cm]{images/embs_vs_users_MLP.png} }}%
    \qquad \qquad \qquad \quad
    \subfloat[\centering \names\ (with privacy-preserving)]{{\includegraphics[width=5.5cm]{images/embs_vs_users_SAL.png} }}%
    \vspace{-2mm}
    \caption{Visualization of representations learned by (a) \textsc{MLP} and (b) \names, which have been reduced to two dimensions via t-SNE and colored by participant identity. Representations learned by \names\ are no longer separable by users which better preserves privacy.\vspace{-4mm}}
    \label{fig:privacy_representations}
\end{figure*}

==> arxiv2021_Mobile Data/figures/tradeoff.tex <==
\begin{figure}%
    \centering
    \vspace{-0mm}
    \includegraphics[width=\linewidth]{images/tradeoff.png}
    \vspace{-4mm}
    \caption{Tradeoff between performance (mood prediction F1 score, \textbf{higher} is better) and privacy (identity prediction accuracy, \textbf{lower} is better). Shaded regions denote standard deviations from the mean (solid lines). \names\ provides a tunable parameter $\sigma$ to control the tradeoff, which allows us to plot a range of (performance, privacy) points. Using a multimodal model on text, keystroke, and app features obtains better performance and privacy at the same time.\vspace{-4mm}}% Incorporating keystrokes, which in itself is the most-privacy preserving feature, brings about boosts in performance while increasing privacy.
    \label{fig:tradeoff}%
\end{figure}

==> arxiv2021_Mobile Data/figures/tsne_combined.tex <==
\begin{figure}%
    \centering
    \subfloat[\centering labels]{{\includegraphics[width=6cm]{images/feat_combined_vs_labels_3.png} }}%
    \qquad
    \subfloat[\centering participant identities]{{\includegraphics[width=6cm]{images/feat_combined_vs_pid.png} }}%
    \caption{Visualization of (Text + Apps) features learned by the \textsc{MLP} model, which have been reduced to two dimensions via t-SNE. Samples are colored by sample by (a) label and (b) participant identity.\vspace{-2mm}}%
    \label{fig:tsne_combined}%
\end{figure}

==> arxiv2021_Mobile Data/tables/MLP_hyperparameters_apps.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{MLP parameter configuration (Apps).}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c}
\Xhline{3\arrayrulewidth}
Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
hidden dim 1 & 128 \\
hidden dim 2 & 128, 64 \\
dropout rate & 0, 0.2, 0.5 \\
learning rate & 0.001 \\
batch size & 100 \\
epochs & 200 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{mlp_params_apps}
\end{table*}

==> arxiv2021_Mobile Data/tables/MLP_hyperparameters_bow.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{MLP parameter configuration (Combined, BoW).}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c}
\Xhline{3\arrayrulewidth}
Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
hidden dim 1 & 1024, 512 \\
hidden dim 2 & 128, 64 \\
dropout rate & 0, 0.2, 0.5 \\
learning rate & 0.001 \\
batch size & 100 \\
epochs & 200 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{mlp_params_bow}
\end{table*}

==> arxiv2021_Mobile Data/tables/SAL_hyperparameters.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{\names\ parameter configuration.}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c}
\Xhline{3\arrayrulewidth}
Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
$\lambda$ & 0.1, 1, 2, 3, 5, 10 \\
$\sigma$ & 1, 5, 10, 25, 50, 100 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{sal_params}
\end{table*}

==> arxiv2021_Mobile Data/tables/SVM_hyperparameters.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{SVM parameter configuration. \\
*Integer kernel values denote the degree of a polynomial kernel.}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c }
\Xhline{3\arrayrulewidth}
Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
C & 0.1, 0.5, 1, 2, 3, 5, 10 \\
Kernel* & RBF, 2, 3, 5, 10 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{svm_params}
\end{table*}

==> arxiv2021_Mobile Data/tables/apps.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table}[t!]
\fontsize{7.5}{11}\selectfont
\centering
\caption{Top $3$ apps associated with positive and negative moods (each row is a different user).\vspace{-2mm}}
\setlength\tabcolsep{2.0pt}
\begin{tabular}{c || c}
\Xhline{3\arrayrulewidth}
Top 3 positive apps & Top 3 negative apps \\
\Xhline{3\arrayrulewidth}
Photos, Settings, Snapchat          & Calendar, Wattpad, SoundCloud \\
FaceTime, MyFitnessPal, Musically   & Notes, App Store, Siri \\
Weather, Phone, FaceTime            & Chrome, App Store, SMS \\
Weather, Phone, Spotify             & Safari, Notes, GroupMe \\
Spotlight, App Store, Uber          & Pinterest, Phone, Yolo \\
Uber, Netflix, LinkedIn             & Phone, Calendar, Safari \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{apps}
\vspace{-4mm}
\end{table}

==> arxiv2021_Mobile Data/tables/emojis.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table}[t!]
\fontsize{8.5}{11}\selectfont
\centering
\caption{Top emojis associated with positive and negative mood (each row is a different user).\vspace{-2mm}}
\setlength\tabcolsep{0.0pt}
\begin{tabular}{c || c}
\Xhline{3\arrayrulewidth}
Positive emojis & Negative emojis \\
\Xhline{3\arrayrulewidth}
\begin{minipage}{.18\textwidth}
    \includegraphics[width=\linewidth]{images/positive.png}
\end{minipage}
&
\begin{minipage}{.22\textwidth}
    \includegraphics[width=\linewidth]{images/negative.png}
\end{minipage}\\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{emojis}
\vspace{-2mm}
\end{table}

==> arxiv2021_Mobile Data/tables/hyperparameters.tex <==
\begin{table*}[t]
\fontsize{9}{11}\selectfont
\centering
\caption{Model parameter configurations. *Integer kernel values denote the degree of a polynomial kernel.}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c | c }
\Xhline{3\arrayrulewidth}
Model & Parameter & Value \\
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{SVM}
& C & 0.1, 0.5, 1, 2, 3, 5, 10 \\
& Kernel* & RBF, 2, 3, 5, 10 \\
\Xhline{0.5\arrayrulewidth}
\multirow{6}{*}{MLP}
& hidden dim 1 (multimodal \& text only) & 1024, 512 \\
& hidden dim 2 (multimodal \& text only) & 128, 64 \\
& hidden dim 1 (keystrokes only) & 64, 32 \\
& hidden dim 2 (keystrokes only) & 32, 16 \\
& hidden dim 1 (apps only) & 128 \\
& hidden dim 2 (apps only) & 128, 64 \\
& dropout rate & 0, 0.2, 0.5 \\
& learning rate & 0.001 \\
& batch size & 100 \\
& epochs & 200 \\
\Xhline{0.5\arrayrulewidth}
\multirow{2}{*}{\names}
& $\lambda$ & 0.1, 1, 2, 3, 5, 10 \\
& $\sigma$ & 1, 5, 10, 25, 50, 100, 150 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{params}
\end{table*}

==> arxiv2021_Mobile Data/tables/modalities_comparison.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
%\vspace{-4mm}
\centering
\caption{Comparison of mood prediction performance across different modalities. Best results in \textbf{bold}. For both accuracy and F1 score, models jointly trained on text, keystroke, and apps features outperform models trained using individual modalities. $\star$ denotes that the difference between multimodal and all unimodal models is statistically significant (p-value $<< 0.05$).\vspace{-2mm}}
\setlength\tabcolsep{5.0pt}
\begin{tabular}{l || c c c c | c c c c }
\Xhline{3\arrayrulewidth}
& \multicolumn{4}{c|}{\textsc{F1 score}} & \multicolumn{4}{c}{\textsc{Accuracy}} \\
Modalities & \textsc{Baseline} & \textsc{SVM} & \textsc{MLP} & \names &  \textsc{Baseline} & \textsc{SVM} & \textsc{MLP} & \names \\
\Xhline{3\arrayrulewidth}
Text + Keystrokes + Apps & $19.07$ & $\textbf{62.81}^{\star}$ & $\textbf{59.61}^{\star}$ & $\textbf{60.11}^{\star}$ & $40.18$ & $\textbf{67.43}^{\star}$ & $\textbf{63.59}^{\star}$ & $\textbf{64.06}^{\star}$\\
Text + Keystrokes & $19.07$ & $61.19$ & $57.65$ & $58.70$ & $40.18$ & $65.87$ & $61.81$ & $62.61$ \\
Text + Apps &  $19.07$ & $62.08$ & $58.38$ & $52.90$ & $40.18$ & $66.59$ & $62.93$ & $56.76$ \\
\Xhline{0.5\arrayrulewidth}
Text & $19.07$ & $61.15 $ & $56.27$ & $52.63$ & $40.18$ & $65.83$ & $60.61$ & $56.08$ \\
Keystrokes & $19.07$ & $57.68$ & $51.43$ & $34.73$ & $40.18$ & $61.03$ & $55.87$
& $39.18$ \\
Apps & $19.07$ & $58.65$ & $52.29$ & $51.32$ & $40.18$ & $62.65$ & $55.26$ & $55.68$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\vspace{-4mm}
\label{modalities_comparison}
\end{table*}

==> arxiv2021_Mobile Data/tables/privacy_data.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{We report user identity prediction performance from raw input data and find that identities are \textbf{very easily revealed} from text, keystrokes, and app usage.\vspace{-2mm}}
\setlength\tabcolsep{5.0pt}
\begin{tabular}{l || c c | c c }
\Xhline{3\arrayrulewidth}
& \multicolumn{2}{c|}{\textsc{F1 score}} & \multicolumn{2}{c}{\textsc{Accuracy}} \\
Modalities & \textsc{SVM} & \textsc{MLP} & \textsc{SVM} & \textsc{MLP} \\
\Xhline{3\arrayrulewidth}
Text & $89.42$ & $92.05$ & $90.60$ & $93.12$ \\
Keystrokes & $91.36$ & $87.04$ & $90.98$ & $87.15$ \\
Apps & $85.68$ & $87.49$ & $90.91$ & $92.00$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\vspace{-4mm}
\label{privacy_data}
\end{table}

==> arxiv2021_Mobile Data/tables/privacy_features.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table}[t!]
\fontsize{8.5}{11}\selectfont
\centering
\caption{Comparison of our privacy-preserving approach (\names) with the baseline (\textsc{MLP}). We evaluate privacy in predicting user identity from learned \textbf{representations} (\textbf{lower} accuracy is better), and find that \names\ effectively obfuscates user identity while retaining performance. T: text, K: keystrokes, A: apps.\vspace{-2mm}}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l || c c | c c}
\Xhline{3\arrayrulewidth}
& \multicolumn{2}{c|}{\textsc{Performance} ($\uparrow$)} & \multicolumn{2}{c}{\textsc{Privacy} ($\downarrow$)}  \\
Modalities & \textsc{MLP} & \names & \textsc{MLP} & \names \\
%& & (best priv) & & (best perf) \\
\Xhline{3\arrayrulewidth}
T + K + A & $59.61$ & $58.48$ & $71.47$ & $\mathbf{34.49}$\\
T + K & $57.65$ & $57.40$ & $64.17$ & $\mathbf{30.99}$ \\
T + A & $58.38$ & $57.76$ & $79.04$ & $\mathbf{65.13}$ \\
T & $56.27$ & $54.11$ & $76.41$ & $\mathbf{52.20}$ \\
K & $51.43$ & $42.48$ & $55.61$ & $\mathbf{25.71}$ \\
A & $52.29$ & $49.15$ & $85.94$ & $\mathbf{66.74}$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{privacy_features}
\vspace{-4mm}
\end{table}

==> arxiv2021_Mobile Data/tables/pvalue_compare_modalities.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{Comparing multimodal to single modalities}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l l || c c | c c }
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{2}{c|}{{Combined $\minus$ Text}} & \multicolumn{2}{c}{{Combined $\minus$ Apps}}  \\
& & $\Delta$ & p-value & $\Delta$ & p-value \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SVM}
& \multirow{1}{*}{accuracy} & $0.75$ & $0.2537$ & $3.93$ & $0.0038$ \\
& \multirow{1}{*}{balanced acc.} & $1.19$ & $0.1206$ & $0.54$ & $0.6768$ \\
& \multirow{1}{*}{average F1} & $0.92$ & $0.1664$ & $3.42$ & $0.0083$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{MLP}
& \multirow{1}{*}{accuracy} & $2.33$ & $0.0095$ & $7.67$ & $0.0025$ \\
& \multirow{1}{*}{balanced acc.} & $1.77$ & $0.0109$ & $4.39$ & $0.0035$ \\
& \multirow{1}{*}{average F1} & $2.11$ & $0.0183$ & $6.09$ & $0.0025$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SAL}
& \multirow{1}{*}{accuracy} & $1.96$ & $0.0463$ & $0.78$ & $0.3994$ \\
& \multirow{1}{*}{balanced acc.} & $1.28$ & $0.1931$ & $1.76$ & $0.2223$ \\
& \multirow{1}{*}{average F1} & $2.45$ & $0.234$ & $-0.10$ & $0.6006$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{pvalue_compare_modalities}
\end{table*}

\iffalse
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{p-value compared modalities (maybe include? really only MLP seems easy to talk about since it's clearly that Combined > BoW > App since they're all statistically significant. not really the case for svm though and def not for SAL)}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l l || c c | c c | c c }
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{2}{c|}{{Combined $\minus$ BoW}} & \multicolumn{2}{c|}{{Combined $\minus$ Apps}} & \multicolumn{2}{c}{{BoW $\minus$ Apps}} \\
& & $\Delta$ & p-value & $\Delta$ & p-value & $\Delta$ & p-value\\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SVM}
& \multirow{1}{*}{accuracy} & $0.75$ & $0.2537$ & $3.93$ & $0.0038$ & $3.18$ & $0.0183$ \\
& \multirow{1}{*}{balanced acc.} & $1.19$ & $0.1206$ & $0.54$ & $0.6768$ & $-0.65$ & $0.6394$ \\
& \multirow{1}{*}{average F1} & $0.92$ & $0.1664$ & $3.42$ & $0.0083$ & $2.50$ & $0.1013$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{MLP}
& \multirow{1}{*}{accuracy} & $2.33$ & $0.0095$ & $7.67$ & $0.0025$ & $5.35$ & $0.0063$ \\
& \multirow{1}{*}{balanced acc.} & $1.77$ & $0.0109$ & $4.39$ & $0.0035$ & $2.62$ & $0.0463$ \\
& \multirow{1}{*}{average F1} & $2.11$ & $0.0183$ & $6.09$ & $0.0025$ & $3.98$ & $0.0142$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SAL}
& \multirow{1}{*}{accuracy} & $1.96$ & $0.0463$ & $0.78$ & $0.3994$ & $-1.18$ & $0.7462$ \\
& \multirow{1}{*}{balanced acc.} & $1.28$ & $0.1931$ & $1.76$ & $0.2223$ & $0.49$ & $0.3994$ \\
& \multirow{1}{*}{average F1} & $2.45$ & $0.234$ & $-0.10$ & $0.6006$ & $-2.54$ & $0.9156$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{pvalue_compare_modalities}
\end{table*}
\fi

==> arxiv2021_Mobile Data/tables/pvalue_compare_to_baseline.tex <==

\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{p-value compared to baseline (seems pretty messy. don't want to include, will just say p-value is significant across all models, features, and metrics)}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l l || c c | c c | c c }
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{2}{c|}{{Combined}} & \multicolumn{2}{c|}{{Text}} & \multicolumn{2}{c}{{Apps}} \\
& & $\Delta$ & p-value & $\Delta$ & p-value & $\Delta$ & p-value\\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SVM}
 & \multirow{1}{*}{accuracy} & $26.41$ & $<0.005$ & $25.65$ & $<0.005$  & $22.47$ & $<0.005$ \\
& \multirow{1}{*}{balanced acc.} & $29.29$ & $<0.005$ & $28.09$ & $<0.005$  & $28.75$ & $<0.005$ \\
& \multirow{1}{*}{average F1} & $43.01$ & $<0.005$ & $42.09$ & $<0.005$  & $39.59$ & $<0.005$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{MLP}
& \multirow{1}{*}{accuracy} & $22.75$ & $<0.005$ & $20.43$ & $<0.005$  & $15.08$ & $<0.005$ \\
& \multirow{1}{*}{balanced acc.} & $28.00$ & $<0.005$ & $26.23$ & $<0.005$  & $23.61$ & $<0.005$ \\
& \multirow{1}{*}{average F1} & $39.31$ & $<0.005$ & $37.20$ & $<0.005$  & $33.22$ & $<0.005$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SAL}
& \multirow{1}{*}{accuracy} & $15.31$ & $<0.005$ & $13.35$ & $<0.005$  & $14.53$ & $<0.005$ \\
& \multirow{1}{*}{balanced acc.} & $22.10$ & $<0.005$ & $20.83$ & $<0.005$  & $20.34$ & $<0.005$ \\
& \multirow{1}{*}{average F1} & $31.36$ & $<0.005$ & $28.92$ & $<0.005$  & $31.16$ & $<0.005$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{pvalue_compare_to_baseline}
\end{table*}

==> arxiv2021_Mobile Data/tables/statistics.tex <==
\begin{table*}[h]
\fontsize{9}{11}\selectfont
\centering
\caption{Mobile Assessment for the Prediction of Suicide (MAPS) dataset summary statistics.}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c | c c c | c }
\Xhline{3\arrayrulewidth}
Users & Datapoints & Modalities & Features & Dimensions & Labels \\
\Xhline{3\arrayrulewidth}
\multirow{3}{*}{$17$} & \multirow{3}{*}{$1641$} & Text & bag-of-words, one-hot & $2000$ & \multirow{3}{*}{Daily mood: negative, neutral, positive}\\
& & Keystrokes & bag-of-timings & $100$\\
& & App usage & bag-of-apps, one-hot & $274$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\vspace{-0mm}
\label{statistics}
\end{table*}

==> arxiv2021_Mobile Data/tables/stb_data_sources.tex <==
\begin{table}[h]
\begin{center}
%\small
%\fontsize{9}{10}\selectfont
\setlength{\tabcolsep}{7.5pt}
%\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|p{30mm}|p{45mm}|p{45mm}|}
\hline
Risk Domain &   Mobile Sensing Data   &   Example Features \\
\hline \hline
Emotional distress  &
Acoustic voice; Sentiment in communication (e.g., social media, text messaging); Facial expression (selfies); Music choice.  &
Fundamental frequency of voice; Positive or negative sentiment in language; Sad or anxious facial expression; Change in music selection.\\
\hline
Social dysfunction (e.g., thwarted belongingness, perceived burdensomeness) &
Self and social content in communication; Patterns of online communication (frequency, diversity of contacts); Geographic movement. &
Negative self-sentiment in language; Bullying or social rejection; Reduction in frequency and diversity of social contacts.\\
\hline
Sleep disturbance (biological diathesis)    &
Actigraphy; Light Sensor, Diurnal Patterns of phone Use.    &
Time in bed; Total sleep time; Sleep onset latency; Wake after sleep onset.\\
\hline
\end{tabular}
\end{center}
%\caption{}
\end{table}

==> arxiv2021_Mobile Data/tables/text_keystrokes.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{Mood prediction using a \textsc{MLP} from text and keystroke features tallied from (1) all characters, (2) a split between types of characters, as well as (3) aggregated across words.\vspace{-2mm}}
\setlength\tabcolsep{5.0pt}
\begin{tabular}{l || c | c c c | c c c | c c c}
\Xhline{3\arrayrulewidth}
Modalities & \textsc{F1 score} & \textsc{Accuracy} \\
\Xhline{3\arrayrulewidth}
Text & $56.27$ & $60.61$ \\
Text + Char keystrokes & $\mathbf{57.65}$ & $\mathbf{61.81}$ \\
Text + Split char keystrokes & $57.32$ & $61.21$ \\
Text + Word keystrokes & $56.46$ & $60.68$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\vspace{-4mm}
\label{text_keystrokes}
\end{table}

==> arxiv2021_Mobile Data/tables/text_lms.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{Mood prediction from text using extended pretrained LM encoders. We find that these models struggle on extremely long contexts of typed text.\vspace{-2mm}}
\setlength\tabcolsep{5.0pt}
\begin{tabular}{l || c | c}
\Xhline{3\arrayrulewidth}
Models & \textsc{F1 score} & \textsc{Accuracy} \\
\Xhline{3\arrayrulewidth}
BoW & $\mathbf{56.27}$ & $\mathbf{60.61}$ \\
BERT & $51.42$ & $58.06$ \\
XLNet & $19.85$ & $42.40$ \\
LongFormer & $19.85$ & $42.40$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\vspace{-4mm}
\label{text_lms}
\end{table}

==> arxiv2021_Mobile Data/tables/training_time.tex <==
\begin{table*}[!tbp]
\fontsize{9}{11}\selectfont
\centering
\caption{Approximate training times (total across $10$-fold cross validation and hyperparameter search).}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c | c }
\Xhline{3\arrayrulewidth}
Model & Modality & Time (hours) \\
\Xhline{3\arrayrulewidth}
\multirow{6}{*}{SVM}
& Text + Keystrokes + Apps & 10 \\
& Text + Keystrokes & 10 \\
& Text + Apps & 10 \\
& Text & 8 \\
& Keystrokes & 1 \\
& Apps & 1 \\
\Xhline{0.5\arrayrulewidth}
\multirow{6}{*}{MLP (100 epochs, 3 runs)}
& Text + Keystrokes + Apps & 6 \\
& Text + Keystrokes & 5 \\
& Text + Apps & 6 \\
& Text & 5 \\
& Keystrokes & 4 \\
& Apps & 2 \\
\Xhline{0.5\arrayrulewidth}
\multirow{1}{*}{\names}
& all & 4 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{times}
\end{table*}

==> arxiv2021_Mobile Data/tables/word_counts.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table*}[t!]
\fontsize{9}{11}\selectfont
\centering
\caption{Top words associated with positive and negative moods across users. We find that while certain positive words are almost always indicative of mood, others are more idiosyncratic and depend on the user.\vspace{-0mm}}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{c c c || c c c}
\Xhline{3\arrayrulewidth}
Positive words & Positive users & Negative users & Negative words & Negative users & Positive users \\
\Xhline{3\arrayrulewidth}
make & 9 & 1 & i'm/im & 10 & 5 \\
yes & 9 & 1 & feel & 7 & 3 \\
got & 7 & 1 & yeah & 7 & 5 \\
still & 7 & 1 & can't/cant & 6 & 2\\
wanna & 7 & 1 & people & 6 & 4 \\
like & 7 & 2 & know & 6 & 4 \\
need & 7 & 2 & go & 6 & 5 \\
send & 7 & 2 & one & 6 & 6 \\
get & 7 & 2 & today & 5 & 1 \\
good & 7 & 3 & day & 5 & 2 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{word_counts}
\vspace{-2mm}
\end{table*}

==> arxiv2021_Mobile Data/tables/word_keystrokes.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table}[t!]
\fontsize{8.5}{11}\selectfont
\centering
\caption{Words with significantly different timings associated with positive and negative moods (each row is a different user).\vspace{-2mm}}
\setlength\tabcolsep{2.0pt}
\begin{tabular}{c || c}
\Xhline{3\arrayrulewidth}
Slower implies positive & Faster implies positive \\
\Xhline{3\arrayrulewidth}
just                                    & why, thank, haha \\
next, was, into, people                 & making, work, idk \\
stuff, cute, phone, want, talk, see     & they, send, dont, man, going \\
don't, talk                             & think, you, all, love \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{word_keystrokes}
\vspace{-4mm}
\end{table}

==> arxiv2021_Mobile Data/tables/words.tex <==
\definecolor{gg}{RGB}{15,125,15}
\definecolor{rr}{RGB}{190,45,45}

\begin{table*}[t!]
\fontsize{9}{11}\selectfont
\centering
\caption{Top 5 words associated with positive and negative moods (each row is a different user).\vspace{-0mm}}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{c || c}
\Xhline{3\arrayrulewidth}
Top 5 positive words & Top 5 negative words \\
\Xhline{3\arrayrulewidth}
hot, goodnight, ft, give, keep      & soon, first, ya, friend, leave \\
still, y'all, guys, new, come       & amazing, see, said, idk, look \\
mind, days, went, tf, next          & tired, hair, stg, snap, anyone \\
girls, music, happy, mean, getting  & omg, people, talking, ask, might \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{words}
\vspace{-2mm}
\end{table*}

==> figures/tsne_combined.tex <==
\begin{figure}%
    \centering
    \subfloat[\centering labels]{{\includegraphics[width=6cm]{images/feat_combined_vs_labels_3.png} }}%
    \qquad
    \subfloat[\centering participant identities]{{\includegraphics[width=6cm]{images/feat_combined_vs_pid.png} }}%
    \caption{Visualization of (Text + Apps) features learned by the \textsc{MLP} model, which have been reduced to two dimensions via t-SNE. Samples are colored by sample by (a) label and (b) participant identity.\vspace{-2mm}}%
    \label{fig:tsne_combined}%
\end{figure}

==> tables/MLP_hyperparameters_apps.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{MLP parameter configuration (Apps).}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c}
\Xhline{3\arrayrulewidth}
Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
hidden dim 1 & 128 \\
hidden dim 2 & 128, 64 \\
dropout rate & 0, 0.2, 0.5 \\
learning rate & 0.001 \\
batch size & 100 \\
epochs & 200 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{mlp_params_apps}
\end{table*}

==> tables/MLP_hyperparameters_bow.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{MLP parameter configuration (Combined, BoW).}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c}
\Xhline{3\arrayrulewidth}
Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
hidden dim 1 & 1024, 512 \\
hidden dim 2 & 128, 64 \\
dropout rate & 0, 0.2, 0.5 \\
learning rate & 0.001 \\
batch size & 100 \\
epochs & 200 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{mlp_params_bow}
\end{table*}

==> tables/SAL_hyperparameters.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{\names\ parameter configuration.}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c}
\Xhline{3\arrayrulewidth}
Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
$\lambda$ & 0.1, 1, 2, 3, 5, 10 \\
$\sigma$ & 1, 5, 10, 25, 50, 100 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{sal_params}
\end{table*}

==> tables/SVM_hyperparameters.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{SVM parameter configuration. \\
*Integer kernel values denote the degree of a polynomial kernel.}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l | c }
\Xhline{3\arrayrulewidth}
Parameter & Value \\
\Xhline{0.5\arrayrulewidth}
C & 0.1, 0.5, 1, 2, 3, 5, 10 \\
Kernel* & RBF, 2, 3, 5, 10 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{svm_params}
\end{table*}

==> tables/pvalue_compare_modalities.tex <==
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{Comparing multimodal to single modalities}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l l || c c | c c }
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{2}{c|}{{Combined $\minus$ Text}} & \multicolumn{2}{c}{{Combined $\minus$ Apps}}  \\
& & $\Delta$ & p-value & $\Delta$ & p-value \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SVM}
& \multirow{1}{*}{accuracy} & $0.75$ & $0.2537$ & $3.93$ & $0.0038$ \\
& \multirow{1}{*}{balanced acc.} & $1.19$ & $0.1206$ & $0.54$ & $0.6768$ \\
& \multirow{1}{*}{average F1} & $0.92$ & $0.1664$ & $3.42$ & $0.0083$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{MLP}
& \multirow{1}{*}{accuracy} & $2.33$ & $0.0095$ & $7.67$ & $0.0025$ \\
& \multirow{1}{*}{balanced acc.} & $1.77$ & $0.0109$ & $4.39$ & $0.0035$ \\
& \multirow{1}{*}{average F1} & $2.11$ & $0.0183$ & $6.09$ & $0.0025$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SAL}
& \multirow{1}{*}{accuracy} & $1.96$ & $0.0463$ & $0.78$ & $0.3994$ \\
& \multirow{1}{*}{balanced acc.} & $1.28$ & $0.1931$ & $1.76$ & $0.2223$ \\
& \multirow{1}{*}{average F1} & $2.45$ & $0.234$ & $-0.10$ & $0.6006$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{pvalue_compare_modalities}
\end{table*}

\iffalse
\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{p-value compared modalities (maybe include? really only MLP seems easy to talk about since it's clearly that Combined > BoW > App since they're all statistically significant. not really the case for svm though and def not for SAL)}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l l || c c | c c | c c }
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{2}{c|}{{Combined $\minus$ BoW}} & \multicolumn{2}{c|}{{Combined $\minus$ Apps}} & \multicolumn{2}{c}{{BoW $\minus$ Apps}} \\
& & $\Delta$ & p-value & $\Delta$ & p-value & $\Delta$ & p-value\\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SVM}
& \multirow{1}{*}{accuracy} & $0.75$ & $0.2537$ & $3.93$ & $0.0038$ & $3.18$ & $0.0183$ \\
& \multirow{1}{*}{balanced acc.} & $1.19$ & $0.1206$ & $0.54$ & $0.6768$ & $-0.65$ & $0.6394$ \\
& \multirow{1}{*}{average F1} & $0.92$ & $0.1664$ & $3.42$ & $0.0083$ & $2.50$ & $0.1013$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{MLP}
& \multirow{1}{*}{accuracy} & $2.33$ & $0.0095$ & $7.67$ & $0.0025$ & $5.35$ & $0.0063$ \\
& \multirow{1}{*}{balanced acc.} & $1.77$ & $0.0109$ & $4.39$ & $0.0035$ & $2.62$ & $0.0463$ \\
& \multirow{1}{*}{average F1} & $2.11$ & $0.0183$ & $6.09$ & $0.0025$ & $3.98$ & $0.0142$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SAL}
& \multirow{1}{*}{accuracy} & $1.96$ & $0.0463$ & $0.78$ & $0.3994$ & $-1.18$ & $0.7462$ \\
& \multirow{1}{*}{balanced acc.} & $1.28$ & $0.1931$ & $1.76$ & $0.2223$ & $0.49$ & $0.3994$ \\
& \multirow{1}{*}{average F1} & $2.45$ & $0.234$ & $-0.10$ & $0.6006$ & $-2.54$ & $0.9156$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{pvalue_compare_modalities}
\end{table*}
\fi

==> tables/pvalue_compare_to_baseline.tex <==

\begin{table*}[!tbp]
\fontsize{8.5}{11}\selectfont
\centering
\caption{p-value compared to baseline (seems pretty messy. don't want to include, will just say p-value is significant across all models, features, and metrics)}
\setlength\tabcolsep{6.0pt}
\begin{tabular}{l l || c c | c c | c c }
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{} & \multirow{2}{*}{} & \multicolumn{2}{c|}{{Combined}} & \multicolumn{2}{c|}{{Text}} & \multicolumn{2}{c}{{Apps}} \\
& & $\Delta$ & p-value & $\Delta$ & p-value & $\Delta$ & p-value\\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SVM}
 & \multirow{1}{*}{accuracy} & $26.41$ & $<0.005$ & $25.65$ & $<0.005$  & $22.47$ & $<0.005$ \\
& \multirow{1}{*}{balanced acc.} & $29.29$ & $<0.005$ & $28.09$ & $<0.005$  & $28.75$ & $<0.005$ \\
& \multirow{1}{*}{average F1} & $43.01$ & $<0.005$ & $42.09$ & $<0.005$  & $39.59$ & $<0.005$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{MLP}
& \multirow{1}{*}{accuracy} & $22.75$ & $<0.005$ & $20.43$ & $<0.005$  & $15.08$ & $<0.005$ \\
& \multirow{1}{*}{balanced acc.} & $28.00$ & $<0.005$ & $26.23$ & $<0.005$  & $23.61$ & $<0.005$ \\
& \multirow{1}{*}{average F1} & $39.31$ & $<0.005$ & $37.20$ & $<0.005$  & $33.22$ & $<0.005$ \\
\Xhline{0.5\arrayrulewidth}
\multirow{3}{*}{SAL}
& \multirow{1}{*}{accuracy} & $15.31$ & $<0.005$ & $13.35$ & $<0.005$  & $14.53$ & $<0.005$ \\
& \multirow{1}{*}{balanced acc.} & $22.10$ & $<0.005$ & $20.83$ & $<0.005$  & $20.34$ & $<0.005$ \\
& \multirow{1}{*}{average F1} & $31.36$ & $<0.005$ & $28.92$ & $<0.005$  & $31.16$ & $<0.005$ \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\label{pvalue_compare_to_baseline}
\end{table*}

==> tables/stb_data_sources.tex <==
\begin{table}[h]
\begin{center}
%\small
%\fontsize{9}{10}\selectfont
\setlength{\tabcolsep}{7.5pt}
%\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|p{30mm}|p{45mm}|p{45mm}|}
\hline
Risk Domain &   Mobile Sensing Data   &   Example Features \\
\hline \hline
Emotional distress  &
Acoustic voice; Sentiment in communication (e.g., social media, text messaging); Facial expression (selfies); Music choice.  &
Fundamental frequency of voice; Positive or negative sentiment in language; Sad or anxious facial expression; Change in music selection.\\
\hline
Social dysfunction (e.g., thwarted belongingness, perceived burdensomeness) &
Self and social content in communication; Patterns of online communication (frequency, diversity of contacts); Geographic movement. &
Negative self-sentiment in language; Bullying or social rejection; Reduction in frequency and diversity of social contacts.\\
\hline
Sleep disturbance (biological diathesis)    &
Actigraphy; Light Sensor, Diurnal Patterns of phone Use.    &
Time in bed; Total sleep time; Sleep onset latency; Wake after sleep onset.\\
\hline
\end{tabular}
\end{center}
%\caption{}
\end{table}
